BiasFinder: Metamorphic Test Generation to Uncover Bias for Sentiment Analysis Systems

Artificial Intelligence (AI) software systems, such as Sentiment Analysis (SA) systems, typically learn from large amounts of data that may reflect human biases. Consequently, the machine learning model in such software systems may exhibit unintended demographic bias based on specific characteristics (e.g., gender, occupation, country-of-origin, etc.). Such biases manifest in an SA system when it predicts a different sentiment for similar texts that differ only in the characteristic of individuals described. Existing studies on revealing bias in SA systems rely on the production of sentences from a small set of short, predefined templates. To address this limitation, we present BisaFinder, an approach to discover biased predictions in SA systems via metamorphic testing. A key feature of BisaFinder is the automatic curation of suitable templates based on the pieces of text from a large corpus, using various Natural Language Processing (NLP) techniques to identify words that describe demographic characteristics. Next, BisaFinder instantiates new text from these templates by filling in placeholders with words associated with a class of a characteristic (e.g., gender-specific words such as female names, "she", "her"). These texts are used to tease out bias in an SA system. BisaFinder identifies a bias-uncovering test case when it detects that the SA system exhibits demographic bias for a pair of texts, i.e., it predicts a different sentiment for texts that differ only in words associated with a different class (e.g., male vs. female) of a target characteristic (e.g., gender). Our empirical evaluation showed that BiasFinder can effectively create a larger number of fluent and diverse test cases that uncover various biases in an SA system.

==> discussion.tex <==
In this section, we show examples of bias-uncovering test cases for each bias, 
analyze the test cases identified as false positive in the user study,
and present threats to validity.

\subsection{Examples of Bias-Uncovering Test Cases}

\ft{The examples need to be updated. The current examples use the old approach.}

\begin{figure}[h]
    {\vspace{-0.5em}}
    \begin{framed}
        \small
        \noindent{\textbf{Original Text}}
        \newline\noindent{Even the trailer for this movie makes me cry, like the first time I saw this movie. Not for people who are easily upset by intense material! The finest performances \textbf{\underline{{\em by Alan Rickman}}} and Madelaine Stowe, without a doubt. This dreadful tale of a society with the power to kidnap and torture it's citizens for ANY reason, whether they are anarchist's or the writer of children's books will chill you to the bone. I saw it when it first came out 1991 and I remember every frame. It still scares the hell out me today. It's happening now. Apparently, IMDb requires ten lines to meet their criteria for a film review. IMDb might want to GET A GRIP! Some of us are a little more succinct about writing opinions.}
        \vspace{0.1cm}\newline\noindent{\textbf{Mutant Text 1}}
        \newline\noindent{Even the trailer for this movie makes me cry, like the first time I saw this movie. Not for people who are easily upset by intense material! The finest performances \textbf{\underline{\em by young Alan Rickman}} and Madelaine Stowe, without a doubt. This dreadful tale of a society with the power to kidnap and torture it's citizens for ANY reason, whether they are anarchist's or the writer of children's books will chill you to the bone. I saw it when it first came out 1991 and I remember every frame. It still scares the hell out me today. It's happening now. Apparently, IMDb requires ten lines to meet their criteria for a film review. IMDb might want to GET A GRIP! Some of us are a little more succinct about writing opinions.}
        \vspace{0.1cm}\newline\noindent{\textbf{SA Prediction for Mutant Text 1}}
        \newline\noindent{Positive}
        \vspace{0.1cm}\newline\noindent{\textbf{Mutant Text 2}}
        \newline\noindent{Even the trailer for this movie makes me cry, like the first time I saw this movie. Not for people who are easily upset by intense material! The finest performances \textbf{\underline{\em by old Alan Rickman}} and Madelaine Stowe, without a doubt. This dreadful tale of a society with the power to kidnap and torture it's citizens for ANY reason, whether they are anarchist's or the writer of children's books will chill you to the bone. I saw it when it first came out 1991 and I remember every frame. It still scares the hell out me today. It's happening now. Apparently, IMDb requires ten lines to meet their criteria for a film review. IMDb might want to GET A GRIP! Some of us are a little more succinct about writing opinions.}
        \vspace{0.1cm}\newline\noindent{\textbf{SA Prediction for Mutant Text  2}}
        \newline\noindent{Negative}
    \end{framed}
    {\vspace{-1em}}
    \caption{Example of BTC for Age}
    \label{fig:example-btc-age}
\end{figure}


\begin{figure}[h]
    {\vspace{-0.5em}}
    \begin{framed}
        \small
        \noindent{\textbf{Original Text}}
        \newline\noindent{There are two things that I noticed in this film. ( This is not a spoiler, just a mistake in storytelling.) When Cole takes Bill to his first B\&E, he finds the " box ". As soon as Cole finds it he says, " The box. Everyone's got a box ". A minute later, just before he dumps the contents on the floor he says, " We're actually very fortunate. You don't see these often ". Observation\# 2 ( Spoiler Alert!) I had to watch the thing three times, I couldn't figure a couple of things out. Then I watched the Chronological version and saw that they were having flash backs from the latter to the previous during the time changes. So at some points we were actually watching three different times in about 1 min of wall time. That was a good thing because I don't know how many more times I could watch it before returning it to Netflix. Color me obsessive.}
        \vspace{0.1cm}\newline\noindent{\textbf{Male Mutant}}
        \newline\noindent{There are two things that I noticed in this film. ( This is not a spoiler, just a mistake in storytelling.) When Cole takes Roen to his first B\&E, he finds the " box ". As soon as Cole finds it he says, " The box. Everyone's got a box ". A minute later, just before he dumps the contents on the floor he says, " We're actually very fortunate. You don't see these often ". Observation\# 2 ( Spoiler Alert!) I had to watch the thing three times, I couldn't figure a couple of things out. Then I watched the Chronological version and saw that they were having flash backs from the latter to the previous during the time changes. So at some points we were actually watching three different times in about 1 min of wall time. That was a good thing because I don't know how many more times I could watch it before returning it to Netflix. Color me obsessive.}
        \vspace{0.1cm}\newline\noindent{\textbf{SA Prediction for Male Mutant}}
        \newline\noindent{Positive}
        \vspace{0.1cm}\newline\noindent{\textbf{Female Mutant}}
        \newline\noindent{There are two things that I noticed in this film. ( This is not a spoiler, just a mistake in storytelling.) When Cole takes Sárinka to her first B\&E, she finds the " box ". As soon as Cole finds it she says, " The box. Everyone's got a box ". A minute later, just before she dumps the contents on the floor she says, " We're actually very fortunate. You don't see these often ". Observation\# 2 ( Spoiler Alert!) I had to watch the thing three times, I couldn't figure a couple of things out. Then I watched the Chronological version and saw that they were having flash backs from the latter to the previous during the time changes. So at some points we were actually watching three different times in about 1 min of wall time. That was a good thing because I don't know how many more times I could watch it before returning it to Netflix. Color me obsessive.}
        \vspace{0.1cm}\newline\noindent{\textbf{SA Prediction for Female Mutant}}
        \newline\noindent{Negative}
    \end{framed}
    {\vspace{-1em}}
    \caption{Example of BTC for Gender}
    \label{fig:example-btc-gender}
\end{figure}

\begin{figure}[h]
    {\vspace{-0.5em}}
    \begin{framed}
        \small
        \noindent{\textbf{Original Text}}
        \newline\noindent{As an earlier reviewer said, Travolta stole every scene he was in. Recognize the character? It was Vinnie Barberino, all grown up and still a bit sleazy, but still likable, oh yes!   Disappointing were William Hurt and Bob Hoskins, perhaps because their characters were badly written, or they just didn't care. I kept seeing one of the Baldwins ( never can remember which) in the Hurt role so Hurt's incredible talents weren't wasted.   Andie McDowell is a sweetie, but not very believable; partly the writing. Character development just wasn't a big thing in this film. Just watch it for Travolta, sit back and enjoy.}
        \vspace{0.1cm}\newline\noindent{\textbf{Mutant Text 1 - Male Name from Greece (Periklis)}}
        \newline\noindent{As an earlier reviewer said, Periklis stole every scene he was in. Recognize the character? It was Vinnie Barberino, all grown up and still a bit sleazy, but still likable, oh yes! Disappointing were William Hurt and Bob Hoskins, perhaps because their characters were badly written, or they just didn't care. I kept seeing one of the Baldwins ( never can remember which) in the Hurt role so Hurt's incredible talents weren't wasted. Andie McDowell is a sweetie, but not very believable; partly the writing. Character development just wasn't a big thing in this film. Just watch it for Periklis , sit back and enjoy}
        \vspace{0.1cm}\newline\noindent{\textbf{SA Prediction for Mutant Text 1}}
        \newline\noindent{Positive}
        \vspace{0.1cm}\newline\noindent{\textbf{Mutant Text 2 - Male Name from Spain (Fransisco Javier)}}
        \newline\noindent{As an earlier reviewer said, Francisco Javier stole every scene he was in. Recognize the character? It was Vinnie Barberino, all grown up and still a bit sleazy, but still likable, oh yes! Disappointing were William Hurt and Bob Hoskins, perhaps because their characters were badly written, or they just didn't care. I kept seeing one of the Baldwins ( never can remember which) in the Hurt role so Hurt's incredible talents weren't wasted. Andie McDowell is a sweetie, but not very believable; partly the writing. Character development just wasn't a big thing in this film. Just watch it for Francisco Javier , sit back and enjoy.}
        \vspace{0.1cm}\newline\noindent{\textbf{SA Prediction for Mutant Text  2}}
        \newline\noindent{Negative}
    \end{framed}
    {\vspace{-1em}}
    \caption{Example of BTC for Country-of-origin}
    \label{fig:example-btc-country}
\end{figure}



\begin{figure}[h]
    {\vspace{-0.5em}}
    \begin{framed}
        \small
        \noindent{\textbf{Original Text}}
        \newline\noindent{" I rented this film because I enjoy watching things with Lauren Graham in them. Well, she was the highlight. Everyone else seemed complete separated from the picture. You kept looking around you at those watching the film with you going, what? However she provided some clarity, as she was the only normal character in the picture, which actually isn't saying much for the film. Personally it was too far fetched for me. However, I am glad I rented despite the fact I would never want to own it. I still feel that Lauren Graham proved to be a strong \textbf{\underline{\em actress}} and even thought she was not the main character, she seemed to steal the movie. My husband and I were happier and cared more about her character ending up with Josh's character than we were about the two main characters. "}
        \vspace{0.1cm}\newline\noindent{\textbf{Mutant Text 1}}
        \newline\noindent{I rented this film because I enjoy watching things with Lauren Graham in them. Well, she was the highlight. Everyone else seemed complete separated from the picture. You kept looking around you at those watching the film with you going, what? However she provided some clarity, as she was the only normal character in the picture, which actually isn't saying much for the film. Personally it was too far fetched for me. However, I am glad I rented despite the fact I would never want to own it. I still feel that Lauren Graham proved to be a strong \textbf{\underline{\em teacher}} and even thought she was not the main character, she seemed to steal the movie. My husband and I were happier and cared more about her character ending up with Josh's character than we were about the two main characters.}
        \vspace{0.1cm}\newline\noindent{\textbf{SA Prediction for Mutant Text 1}}
        \newline\noindent{Positive}
        \vspace{0.1cm}\newline\noindent{\textbf{Mutant Text 2}}
        \newline\noindent{b " I rented this film because I enjoy watching things with Lauren Graham in them. Well, she was the highlight. Everyone else seemed complete separated from the picture. You kept looking around you at those watching the film with you going, what? However she provided some clarity, as she was the only normal character in the picture, which actually isn't saying much for the film. Personally it was too far fetched for me. However, I am glad I rented despite the fact I would never want to own it. I still feel that Lauren Graham proved to be a strong \textbf{\underline{\em lawyer}} and even thought she was not the main character, she seemed to steal the movie. My husband and I were happier and cared more about her character ending up with Josh's character than we were about the two main characters. "}
        \vspace{0.1cm}\newline\noindent{\textbf{SA Prediction for Mutant Text  2}}
        \newline\noindent{Negative}
    \end{framed}
    {\vspace{-1em}}
    \caption{Example of BTC for Occupation}
    \label{fig:example-btc-age}
\end{figure}



\begin{figure}[h]
    {\vspace{-0.5em}}
    \begin{framed}
        \small
        \noindent{\textbf{Original Text}}
        \newline\noindent{In this episode, \underline{\textbf{\textit{a man}}} and \textbf{his} dog go 'coon huntin' after eating dinner with \textbf{his} wife of 50 years. \textbf{He}'s devoted to \textbf{his} wife and \textbf{his} dog. While hunting, \textbf{his} dog jumps in the river after the dog and \textbf{he} follows. \textbf{The man} dies and doesn't know it. \textbf{He} tries to talk to \textbf{his} wife and \textbf{his} grave diggers to no avail.}
        \vspace{0.1cm}\newline\noindent{\textbf{Mutant Text}}
        \newline\noindent{In this episode, \underline{\textbf{\textit{a man}}} and \textbf{her} dog go 'coon huntin' after eating dinner with \textbf{her} wife of 50 years. \textbf{She}'s devoted to \textbf{her} wife and \textbf{her} dog. While hunting, \textbf{her} dog jumps in the river after the dog and \textbf{she} follows. \textbf{The woman} dies and doesn't know it. \textbf{She} tries to talk to \textbf{her} wife and \textbf{her} grave diggers to no avail.}
    \end{framed}
    {\vspace{-1em}}
    \caption{Example of Incorrect Semantic Mutant Found While Doing User Study Triggered by Coreference Resolution Library Capability}
    \label{fig:example-incorrent-semantic}
\end{figure}

\subsection{Analysis of the False Positives from the Survey}

\ft{Need to put examples of false positives from the survey}


\subsection{Threats to Validity}
\vspace{0.2cm}\noindent\textbf{Threats to Internal Validity.} There are some randomness involved in our experiments. We randomly select names for filling placeholders in gender and country-of-origin templates. We also randomly select BTCs for our survey. The results may be different if we have picked a different set of names or BTCs. We minimize these threats by picking unique names across country-of-origin and gender; and picking a high yet reasonable number of BTCs to label. These unique names should cover a large variety of people names and our experiments showed that they can be used to generate a large number of BTCs, showing the ability of \toolname{} to uncover bias (which is the goal of our work). Also, labelling BTCs involves reading a long piece of movie review text and it may take a long time to decide both the coherence and the sentiment of the text. Due to limited manpower and resources, we can only label a limited number of texts.

\vspace{0.2cm}\noindent\textbf{Threats to External Validity.} We have only experimented with SA system based on BERT and generate templates from IMDB dataset. The results may not be generalizable to other SA systems and dataset. However, BERT is one of the top performing models for text classification in recent years~\cite{brown2020language,raffel2019exploring,yang2019xlnet,devlin2019bert}. Also, IMDB dataset is a common dataset used for sentiment analysis~\cite{thongtan2019sentiment,sachan2019revisiting,howard2018universal}. Thus, we believe the threats are minimal as we show that the bias occurs on mutants of texts from a common dataset and the bias is exhibited by one of the top models.

==> exp-comment.tex <==
In this section, we describe our dataset and experimental settings, evaluation metric, and some research questions. We then answer the research questions.
\subsection{Dataset and Experimental Settings}

We focus on a binary sentiment analysis task, i.e., a task of classifying whether a text conveys a positive or a negative sentiment. 
We focus on a binary operationalization of sentiment as bias is associated with a positive or negative point of view, and a sentence with a neutral sentiment will not produce a bias.
A popular dataset to evaluate a sentiment analysis system's performance for this task is the IMDB Dataset of 50K Movie Reviews\cite{maas-EtAl:2011:ACL-HLT2011}. It contains a set of 50,000 movie reviews; each review is labelled as either having an overall positive or negative sentiment. Some of these movie reviews contain texts that are not natural language, e.g., HTML tags. We remove these texts from the movie reviews. We then split the 50,000 movie reviews evenly to train and test sets. 

We use a Transformer-based model as the sentiment analysis system in our experiments. Transformer-based models have achieved state-of-the-art performances on many NLP tasks in recent years~\cite{}\dl{Missing reference}. We pick BERT~\cite{devlin2019bert} as a representative model. It is not our goal to evaluate and compare bias over all sentiment analysis systems -- we leave such extensive comparative evaluation for future work.

BERT is a pre-trained language model that can be {\em fine-tuned} to solve many downstream NLP tasks. We fine-tune BERT for binary sentiment analysis following Sun et al. work~\cite{sun2019fine} and use the implementation they provide.\footnote{\url{https://github.com/xuyige/BERT4doc-Classification}} We fine-tune the BERT sentiment analysis (SA) model using the train set and use the test set as input for Gender\toolname{} to generate mutants.

We performed our experiments on a computer running Ubuntu 18.04 with Intel(R) Core(TM) i7-9700K CPU @ 3.60GHz processor, 64GB RAM, and NVIDIA GeForce RTX 2080. For coreference resolution, we use NeuralCoref\footnote{\url{https://github.com/huggingface/neuralcoref}}. We use both SpaCy\footnote{\url{https://spacy.io/}} and Stanford CoreNLP\footnote{\url{https://stanfordnlp.github.io/CoreNLP/}} for Part-of-Speech (PoS) Tagging and Named Entity Recognition (NER). The syntactic check is performed using   LanguageTool\footnote{\url{https://github.com/languagetool-org/languagetool}}. We built a local server to serve API request of LanguageTool using docker wrapped by DockerLanguageTool\footnote{\url{https://github.com/silvio/docker-languagetool}}.


% \dl{Add text preprocessing here? As the text preprocessing is specific to the IMDB dataset.}
% \mh{addded} 

% \vspace{0.2cm}\noindent {\bf Text Preprocessing for IMDB Moview Review}

% \dl{Description here must be updated.} \mh{updated by me and Yusuf} \dl{I'm afraid the text is still unclear; Ferdian maybe you can work on this as you know the low level details better than I do :-)}
% The {\em Text Processing} receives as an input a collection of texts. The {\em Text Processing Engine} processes the texts one-by-one. 

%\dl{This is still unclear, what do we mean by special tags, why are they meaningless, why are they there in the first place, what do you mean as normal text?} \mh{edited - taken from approach} 

%The movie review texts sometimes contain meaningless tokens (i.e. HTML Tag) for Sentiment Analysis. \toolname{} remove any HTML Tag using regular expression (RegEx).  NLP tasks (such as dependency parsing and coreference resolution) relies on tokenization and tokenization process in English texts relies on punctuation and white-space~\cite{palmer2000tokenisation}. Thus, in this {\em Text Preprocessing}, the original text is cleaned by restructuring the text punctuation. Restructuring process is done by adding a white-space after a stop words punctuation (e.g: a period mark (“.”), question mark (“?”), and exclamation mark (“!”)).  
%Overall, there are 2 techniques in The {\em Text Preprocessing}. i.e., removing HTML Tags and restructuring the punctuation.
%The resulted text from The {\em Text Preprocessing} is shown at Figure~\ref{fig:example-text-preprocessing}.

% \begin{figure}[h]
%     {\vspace{-0.5em}}
%     \begin{framed}
%         \small
%         \noindent{\textbf{Original Text}}
%         \newline\noindent{The cast played Shakespeare.$<$br /$><$br /$>$Shakespeare lost.$<$br /$><$br /$>$I appreciate that this is trying to bring Shakespeare to the masses, but why ruin something so good.$<$br /$><$br /$>$Is it because 'The Scottish Play' is my favorite Shakespeare? I do not know.}
%         \vspace{0.1cm}\newline\noindent{\textbf{After Removing HTML Tags}}
%         \newline\noindent{The cast played \textbf{Shakespeare.Shakespeare} \textbf{lost.I} appreciate that this is trying to bring Shakespeare to the masses, but why ruin something so \textbf{good.Is} it because 'The Scottish Play' is my favorite Shakespeare? I do not know.}
%         \vspace{0.1cm}\newline\noindent{\textbf{After Restructuring The Punctuation}}
%         \newline\noindent{The cast played \textbf{Shakespeare. Shakespeare} \textbf{lost. I} appreciate that this is trying to bring Shakespeare to the masses, but why ruin something so \textbf{good. Is} it because 'The Scottish Play' is my favorite Shakespeare? I do not know.}
%     \end{framed}{\vspace{-1em}}
%     \caption{Example of a Cleaned Text in The {\em Text Processing}}
%     \label{fig:example-text-preprocessing}
% \end{figure}


\subsection{Evaluation Metric}

We measure fairness of SA systems using the number of bias-uncovering test cases (BTCs). A bias-uncovering test case is a pair of mutants generated from a bias-targeting template differing in their class (e.g. male and female) of the demographic characteristic (e.g. gender) that should have the same sentiment, but are labelled with a different sentiment by the SA system. 

% \begin{itemize}[nosep,leftmargin=*]
%     \item {\em Number of bias-uncovering test cases (BTC).} We define a bias-uncovering test case as a pair of sentences that belongs to the same bias-targeting template but produces a different sentiment. 
%     \item{\em Equality Differences (ED).} ED has been used to evaluate bias in text classification~\cite{dixon2018measuring,park2018reducing,garg2019counterfactual}. We measure both False Positive Equality Difference (FPED) and False Negative Equality Difference (FNED):
%     \[
%         FPED = \sum_{p \in P} |  FPR - FPR_p |
%     \]
%     \[
%         FNED = \sum_{p \in P} |  FNR - FNR_p |
%     \]
%     where $p$ indicates a characteristic value (e.g., male), $P$ indicates a characteristic (e.g., gender and age), $FPR$ indicates a false positive rate for the entire testing data, $FNR$ indicates a false negative rate for the entire testing data, $FPR_p$ indicates a false positive rate for texts in the testing data that belongs to characteristic value $p$, and  $FNR_p$ indicates a false negative rate for texts in the testing data that belongs to characteristic value $p$.
% \end{itemize}


\subsection{Research Questions}

\dl{RQ1: Compare the BTCs?}
\dl{RQ2: See if the BTCs detected by our approach {\bf subsumes} those detected by EEC and vice versa.

200k BTCs detected by GenderBiasFinder.
-> debias using EEC (BTCs)
How many percent is left from the 200k? We want to report this percentage. 

[Only y\% of the BTCs detected by GenderBiasFinder is subsumed by EEC BTCs; y = 2\%]

6k BTCs detected by EECs
-> debias using GenderBiasFinder (BTCs)
How many percent is left from the 6k? We want to report this percentage.

[Almost all / All of the BTCs detected by EEC are subsumed by GenderBiasFinder's BTCs]

[Conclusion] Bias detected by GenderBiasFinder is a much larger superset of those detected by EECs.
}

\dl{RQ3: See the number of false positives. Statistically representative sample: 300+. False positive rate: 10\%.}

\dl{Discussion section:
- Number of BTCs detected
- Number of false positives (sample; x need to be statistically representative if you have don't have time; provided that the results are similar to the answer of RQ3)}


\vspace{0.2cm}\noindent\textbf{RQ1. } {\em How is Gender\toolname{} performance compared to the baseline?}
% \vspace{0.2cm}\noindent\textbf{RQ1. } {\em Does having more templates help to uncover more bias?}

%\noindent \textit{How the performance of EEC mutants and \toolname{}'s mutants after debiasing?}

Gender\toolname{} is the first approach that automatically generates templates for uncovering gender bias. We compare the performance of Gender\toolname{} against a baseline of handcrafted templates. We introduced the baseline (i.e., EEC) in Section~\ref{subsec:eec} and use 140 templates described there. Each of these templates has a $\langle person\rangle$ placeholder, which we fill with the same set of names used to generate mutants  in Gender\toolname{}. We report the number of generated mutants by both EEC and Gender\toolname{}. After we get the mutants, we label the mutants with sentiments predicted using the BERT SA model. We then report the BTCs produced by EEC and Gender\toolname{}.

%\dl{I think we can show the number of BTCs too. But we can add more experiments to show if the bias that are detected by one method subsumes the other or not. We may want to split this RQs into two. The first one just the number of BTCs. The second to see if the BTCs covered by one method can cover the other or not.} 

% We debias the BERT SA model from the bias discovered by EEC by training the model using EEC mutants. We report the number of BTCs that can be generated by Gender\toolname{} before and after debiasing the SA model. Similarly, to debias the model from the bias discovered by Gender\toolname{}, we train the model using Gender\toolname{} mutants. We then report the number of BTCs that can be generated by EEC before and after debiasing the SA model. We analyze the reported numbers to compare the performance of Gender\toolname{} and EEC.\ft{Possibly need to change this. The results show that using the whole mutants hurt accuracy too much. Probably better to train using less mutants or only BTCs.}\dl{I haven't checked this paragraph as I don't know if this one is final or not ...}

% \vspace{0.2cm}\noindent\textit{Experimental Procedure}

% \noindent There are 4 different experimental settings:
% \begin{enumerate}
%     \item Fine-tune using 50\% EEC mutants, predict using remaining 50\% EEC mutants
%     \item Fine-tune using 3 EEC templates, predict using 4 remaining template
%     \item Fine-tune using 50\% \toolname{} mutants, predict using remaining 50\% \toolname{} mutants
%     \item Fine-tune using 2000 \toolname{}'s templates, predict using 2002 remaining template
% \end{enumerate}



%\noindent We compare the FPED, FNED, and number of BTC for each setting.

% \noindent \textit{Can \toolname{} find bias that EEC cannot find?} \textit{Can \toolname{} find bias that EEC can find?}
%  Inspired from Park et al \cite{park2018reducing}, we take advantage from fine-tuning to debias the baseline (EEC).
% The previous work by EEC (Section~\ref{subsec:eec}) uses a simple template in generating mutant texts. In this RQ, we want to prove that wide-variety of templates help to find more bugs. We want to demonstrate that \toolname{}'s mutants can find bias that EEC can not find. We also wanto demonstrate that \toolname{}'s mutants can find bias that EEC can find.
% We want to demonstrate that \toolname{}'s mutants can uncover more bias than EEC.

% \vspace{0.2cm}\noindent\textit{Experimental Procedure}

% There are 2 different experimental settings:
% \begin{enumerate}
%     \item Fine-tune using EEC mutants, predict using \toolname{} mutants
%     \item Fine-tune using \toolname{} mutants, predict using EEC mutants
% \end{enumerate}

% \noindent We compare the FPED, FNED, and number of BTC for each setting.

%\dl{Can our approach finds bias that EEC can find? Our experiment only shows that our approach can find bias that EEC cannot find.} \dl{Maybe you can use the biases that you find using your tool BiasFinder to train a new model and see if the templates generated by EEC can still detect those biases? Maybe the number of discordant pairs are reduced?}


\vspace{0.2cm}\noindent\textbf{RQ2.} {\em Does the BTCs detected by Gender\toolname{} {\bf subsumes} those detected by EEC?}

\mh{edited} In the RQ1, we calculate the number of BTCs produced by EEC and Gender\toolname{}. To compare the performance of EEC and \toolname{} templates in discovering gender bias, we cannot simply count the number of BTCs, as the BTCs discovered from the two set of templates may cover the same bias. To check if Gender\toolname{} discovers a different bias, we first need to debias the target BERT SA model from the bias discovered by EEC. One can debias a BERT SA model by fine-tuning the model using a debiased dataset~\cite{park2018reducing}. \dl{Training is a wrong word here. We are not training, we are only fine-tuning.}
\mh{replace the fine-tuning definition}  Fine-tuning the model is achieved by (1) freezing the BERT feature extraction layer that capture semantic and syntactic information , and (2) updating subsequent layers using a small number of learning rate. Intuitively, the lower layer of the BERT model may contain more general information\cite{sun2019fine}. We fine-tune the BERT SA model using a set of mutants with the correct sentiment labels (i.e., the ground truth sentiment labels of the original texts used to generate the templates). 

% \dl{I don't quite understand this, I though GenderBiasFinder uses more names from GenderComputer. When GenderBiasFinder uses more names and when does it use less names? I'm not sure} To control for the effects of different placeholder values, we use the same set of person names for $\langle name \rangle$ placeholder values when generating mutants using EEC and \toolname{} templates. The set of person names are taken from EEC as we want to keep EEC as is.

We want to check the BTCs correlation between EEC and Gender\toolname{}. Does the BTCs from Gender\toolname{} covers the BTCs from EEC and vice versa? To do that, we debias the BERT SA model from the bias discovered by EEC by fine-tuning the model using ECC BTCs. We report the number of BTCs that can be generated by Gender\toolname{} after debiasing the SA model using EEC BTCs. Similarly, to debias the model from the bias discovered by Gender\toolname{}, we fine-tune the model using Gender\toolname{} BTCs. We then report the number of BTCs that can be generated by EEC after debiasing the SA model using Gender\toolname{} BTCs. We alo report the percentage of BTCs left after debiasing. We analyze the reported numbers to compare the performance of Gender\toolname{} and EEC.

\mh{added} To avoid an overfitting problem when fine-tuning, we only select a unique mutant from BTCs. For example if we have 3 BTCs: $(m_{1}, m_{2})$ and $(m_{1}, m_{3})$, $(m_{1}, m_{4})$ while $m_{i}$ represent mutant $ \mathit{i}$-th. Thus, we only fine-tune using a set of unique mutants $[m_{1}, m_{2}, m_{3}, m_{4}]$. \mh{Hi Prof David, Ferdian and Hongjin, do you agree with this argument? I'm still running the experiment to see the result if we use the whole BTCs}


\begin{comment}

200k BTCs detected by GenderBiasFinder.
-> debias using EEC (BTCs)
How many percent is left from the 200k? We want to report this percentage. 

[Only y\% of the BTCs detected by GenderBiasFinder is subsumed by EEC BTCs; y = 2\%]

6k BTCs detected by EECs
-> debias using GenderBiasFinder (BTCs)
How many percent is left from the 6k? We want to report this percentage.

[Almost all / All of the BTCs detected by EEC are subsumed by GenderBiasFinder's BTCs]

\end{comment}

% \vspace{0.2cm}\noindent\textbf{RQX. } {\em Does having more placeholder values help to uncover more biases?}

% \noindent We want to know how much placeholder values matter when generating mutants from templates. We experiment with generating mutants using only a subset of values (e.g., 20\%, 40\%, etc.). We then debias the BERT SA model using the generated mutants. We test the debiased model on mutants generated using the remaining set of values. If we cannot find any BTCs from these mutants, it suggests that it is not necessary to generate mutants using all the values. It is sufficient to generate mutants using only a subset of the values.  \mh{make variations: (1) fine-tune with template, (2) fine-tune with template + 10\% mutant ..... increase 10\% until get 0 BTC}

% \begin{comment}
%     \noindent \mh{The setting looks odd, skip this RQ} In the previous research question, we want to uncover that wide-variety of templates help to find bugs. Complementing the previous research question, we want to see whether the wide-variety of place-holder value help to find bugs. We use EEC template to check this. We substitute each person placeholder with lots number of name obtained from GenderComputer\footnote{\url{https://github.com/tue-mdse/genderComputer}}. 
    
    
    
%     \vspace{0.2cm}\noindent\textit{Mutant Generation for RQ2} \mh{the pipeline looks odd}
    
%     \begin{enumerate}
%         \item Prepare list of templates from EEC 
%         \item Prepare name from GenderComputer. We only pick 310 names come from 31 different countries. 10 sentences from each country with 5 male names and 5 female names.
%         \item Mutant generation by substituting name from GenderComputer to EEC template
%     \end{enumerate}
    
%     \vspace{0.2cm}\noindent\textit{Experimental Procedure for RQ2}
    
%     \begin{enumerate}
%         \item Prepare generated mutant into male and female test data. We need to differentiate male and female data to calculate FPED, FNED, and number of discordant pairs.
%         \item Prepare BERT classification task fine-tuned using IMBD movie review
%         \item Fine-tune model again using original EEC data 
%         \item Predict using generated mutant for RQ3
%         \item Measure the FPED, FNED, and number of discordant pairs 
%     \end{enumerate}
    
%     In this experimental setting, we fine-tune using original EEC to know that after debias the model using EEC original data, can we still find a bug by adding more value for name? 
% \end{comment}



%\vspace{0.2cm}\noindent\textbf{RQ3. }{\em How good is Gender\toolname{} in generating bias-uncovering test cases?}

%\noindent We report the number of BTCs that can be generated for gender bias. \dl{What is the difference between this and RQ1?}  %We also measure FPED and FNED for each of these biases. In this experiment we fine-tune the BERT-model using IMDB train data on 1 epoch. We generate mutant using IMDB test data. Then we predict the sentiment of generated mutant using fine-tuned BERT. For each \characteristic we present the number of BTC, FPED, and FNED.

%\vspace{0.2cm}\noindent\textbf{RQ4. } {\em Does selecting bias-uncovering values help in accelerating the generation of bias-uncovering test cases?}

\noindent 

%\vspace{0.2cm}\noindent\textbf{RQ5. } {\em How effective is the two-stage filtering approach in removing semantically incorrect mutant texts?}

\noindent 

\vspace{0.2cm}\noindent\textbf{RQ3. }{\em How many false positives bias-uncovering test  cases from Gender\toolname{} are there? }

\noindent We measure the quality of the generated mutant texts and bias-uncovering test cases via a survey. The survey involves \ft{fill in} participants and \ft{fill in} statistically representative sample mutant texts. \dl{We shouldn't use the word quality. We need to be more explicit, e.g., by using the term ``false positives'', etc.}

%\vspace{0.2cm}\noindent\textbf{RQ7. }{\em Can we use the generated mutant texts to guide the repair of biased sentiment prediction in the original text? }


%\dl{We need to do ablation studies later to show the impact of omitting some of these steps.}\ft{These are already included in RQs. We can make this clearer.}

\subsection{Results}

\vspace{0.2cm}\noindent\textbf{RQ1. } {\em Gender\toolname{} Comparison with Baseline}

\begin{comment}
    \begin{table}[H]
        \centering
        \caption{Performance of EEC and \toolname{} after Debiasing \mh{maybe we can try to see another thing by changing the \% of train test}}
        \begin{tabular}{ clcccc }
        \hline
        \textbf{No} & \textbf{Fine-Tune Data} & \textbf{Test Data} & \textbf{FPED} & \textbf{FNED} & \textbf{\# BTC} \\
        \hline
        1 & 50\% EEC & 50\% remaining & 0 & 0 & 0 \\
        % 2 & 4 EEC templates & 3 EEC & 0 & 0 & 0 \\
        2 & 50\% \toolname{} & 50\% remaining & 0 & 0 & 0 \\
        % 4 & 6/7 EEC & \toolname{} mutant & 0.000201 & 0.005645 & 13,922 \\
        \hline
        % \multicolumn{6}{l}{BTC: Bias-uncovering Test Cases}\\
        \end{tabular}
        \label{tab:rq2}
    \end{table}
    The results show that since the EEC template is too simplistic, debiasing the template is relatively easy. \mh{I plan to decrease the number of fine-tune data to see another result}
    \dl{For Table IV, I don't know if the result is as expected. Our approach should generate a more diverse set of templates than EEC right? So if we train using half of the templates, and test using the other half, then shouldn't we get a non-zero BTC? If we get a zero BTC, reviewers will ask, what's the point of getting 300k BTC, when only a small subset can block the rest?}\ft{This experiment is not yet done. Table 4 was reporting a different thing (taking random mutants rather than picking some of the templates). We will put the results of diverse templates experiments in Table 4 when we get them. Should we have another experiment where we use some templates from \toolname{} to debias SA model and check if the other templates still lead to BTCs? }

\end{comment}

%\dl{If I don't fine tune using EEC, how many BTCs can I find using BiasFinder? If I don't fine tune using BiasFinder, how many BTCs can I find using EEC? One result could be that EEC does not help BiasFinder, but BiasFinder, can help reduce EEC bias. We can also show that the approaches are complementary.}

\begin{table}[H]
    \centering
    \caption{Mutant Statistics}
    \begin{tabular}{ lccccc}
    \hline
    \textbf{Data} & \textbf{\# Templates} & \textbf{\# Male } & \textbf{\# Female }  & \textbf{\# Total } \\
    \hline
    EEC & 140 & 4,200 & 4,200 & 8,400 \\
    Gender\toolname{} & 3,730 & 493,376 & 493,376 & 986,752 \\
    \hline
    \end{tabular}
    \label{tab:mutant-statistic}
\end{table}

Table~\ref{tab:mutant-statistic} shows the number of mutants generated by EEC and Gender\toolname{} % using the set of names taken from EEC.
Gender\toolname{} discovered a lot of templates automatically and produces 986,752 mutants from them, much larger than the number of mutants generated by EEC, i.e., 8,400 mutants. 

\begin{table}[H]
    \centering
    \caption{Comparison of The BTCs produced by EEC and \toolname{}}
    \begin{tabular}{ lc }
    \hline
    \textbf{} & \textbf{\# BTC} \\
    \hline
    EEC & 16,868 \\
    Gender\toolname{} & 71,027 \\
    \hline
    \end{tabular}
    \label{tab:btc-comparison}
\end{table}

Table~\ref{tab:btc-comparison} shows the number of BTCs that are generated by EEC and Gender\toolname{}.
 



% Table~\ref{tab:rq2} shows the number of BTCs that can be generated by EEC and Gender\toolname{} before and after debiasing. It shows that, if we debias the target SA model by training the model on the 8,400 EEC mutants, Gender\toolname{} can still find 3,536 BTCs, which are only 103 BTCs less from 3,639 BTCs that can be found for the model has not been debiased from the bias discovered by EEC. This suggest that the bias discovered by EEC only covers a subset of bias discovered by Gender\toolname{}.

% Table~\ref{tab:rq2} also shows that, if we debias the target SA model by training the model on the 140,842 Gender\toolname{} mutants, there are no BTCs that can be generated from EEC mutants, suggesting that the bias discovered by Gender\toolname{} actually covers the bias discovered by EEC. These results suggest that Gender\toolname{} is better than EEC in discovering bias in sentiment analysis system.


% \begin{table*}[h]
%     \centering
%     \caption{Bias-uncovering Test Cases (BTCs) of EEC and Gender\toolname{} using Mutants in Table~\ref{tab:mutant-statistic-rq1} }
%     \begin{tabular}{ clccc}
%     \hline
%     \textbf{1st Fine-tune} & \textbf{2nd Fine-tune} & \textbf{Test Data} & \textbf{\# BTC 1st Fine-Tune} & \textbf{\# BTC 2nd Fine} \\
%     \hline
%     IMDB train & EEC & Gender\toolname{} & 3,639 & 3,536 \\
%     IMDB train & Gender\toolname{} & EEC & 6,390 & 0 \\
%     \hline
%     %\multicolumn{6}{l}{BTC: Bias-uncovering Test Cases}\\
%     \end{tabular}
%     \label{tab:rq2}
% \end{table*}


\begin{comment}
\begin{table}[h]
    \centering
    \caption{Comparison of Bias-uncovering Performance of EEC and Gender\toolname{} }
    \begin{tabular}{ clcccc }
    \hline
    \textbf{No} & \textbf{Fine-Tune Data} & \textbf{Test Data} & \textbf{FPED} & \textbf{FNED} & \textbf{\# BTC} \\
    \hline
    1 & EEC & \toolname{} & 0.00013 & 0.00525 & 6,844 \\
    2 & \toolname{} & EEC & 0.00761 & 0.00063 & 3,620 \\
    \hline
    %\multicolumn{6}{l}{BTC: Bias-uncovering Test Cases}\\
    \end{tabular}
    \label{tab:rq2}
\end{table}

\end{comment}

% \dl{For Table 5, BiasFinder has much more mutants than EEC right? By right, BiasFinder should find much more BTC than EEC right? So why the BTC numbers for the two cases are more or less the same? Does it mean that BiasFinder is not as effective as EEC?}


\begin{comment}
\vspace{0.2cm}\noindent\textbf{RQ1. } {\em Gender\toolname{} Comparison with Baseline}

\begin{table}[H]
    \centering
    \caption{RQ1}
    \begin{tabular}{ clcccc }
    \hline
    \textbf{No} & \textbf{Fine-Tune Data} & \textbf{Test Data} & \textbf{FPED} & \textbf{FNED} & \textbf{\# BTC} \\
    \hline
    1 & 95\% EEC data & 5\%EEC & 0 & 0 & 0 \\
    2 & 95\% EEC data & \toolname{} mutant & 0.00140 & 0.00326 & 12,342 \\
    3 & 6/7 EEC & 1/7 EEC & 0 & 0 & 0 \\
    4 & 6/7 EEC & \toolname{} mutant & 0.000201 & 0.005645 & 13,922 \\
    \hline
    \multicolumn{6}{l}{BTC: Bias-uncovering Test Cases}\\
    \end{tabular}
    \label{tab:rq2}
\end{table}

Table~\ref{tab:rq2} shows that EEC templates is too simplistic. (1) and (3) are settings that are intended to know the effect of fine-tuning on EEC data. (2) and (4) are settings that are intended to know the effect of fine-tuning on our generated mutant. From (1) and (3), all evaluation metrics (FPED, FNED, and number of discordant pairs) are 0, which means after debiasing model by fine-tuning, EEC template can't produce bugs in the debiased model. From (2) and (4), all evaluation metrics are non zero, which means after debiasing model by fine-tuning, our mutant produce bugs in the debiased model.    

\end{comment}


\vspace{0.2cm}\noindent\textbf{RQ2. } {\em Does the BTCs detected by \toolname{} {\bf subsumes} those detected by EEC and vice versa?}

\begin{table*}[h]
    \centering
    \caption{Comparison of The BTCs After Debiasing}
    \begin{tabular}{ llcc }
    \hline
    \textbf{Testing Tool} & \textbf{Debiasing Data} & \textbf{\# BTC After Debiasing} & \textbf{\% BTC Left} \\
    \hline
    EEC & Augmented (IMDB + Unique Mutants from BTCs by Gender\toolname{}) & 7,639 & 44\% \\
    EEC & Augmented(IMDB + Full Mutants from BTCs by Gender\toolname{}) & - & -\% \\
    EEC & Full Mutants from BTCs by Gender\toolname{} & - & -\% \\
    Gender\toolname{} & Augmented (IMDB + Unique Mutants from BTCs by EEC) & 13,295 & 19\% \\
    Gender\toolname{} & Augmented (IMDB + Full Mutants from BTCs by EEC) & - & -\% \\
    Gender\toolname{} & Full Mutants from BTCs by EEC & 656 & -\% \\
    \hline
    \end{tabular}
    \label{tab:debiasing-effect}
\end{table*}



% \vspace{0.2cm}\noindent\textbf{RQX. } {\em Does having more placeholder values help to uncover more bias?}

% \begin{table}[H]
%     \centering
%     \caption{The Effect of Value-placeholder Replacement in Debiasing}
%     \begin{tabular}{ lcc }
%     \hline
%     \textbf{Fine-tune Data} & \textbf{Test Data} & \textbf{\# BTC}\\
%     \hline
%     Original Texts + 0\% Mutants & 100\% Mutants & 53,122 \\
%     Original Texts + 20\% Mutants & 80\% Mutants & - \\
%     Original Texts + 40\% Mutants & 60\% Mutants & - \\
%     Original Texts + 60\% Mutants & 40\% Mutants & 0 \\
%     \end{tabular}
%     \label{tab:rq3}
% \end{table}

% Table~\ref{tab:rq3} shows that all evalutaion metric is 0. This indicate that BERT fine-tuning model is good for handling diverse values from the generated mutant. After fine-tuning using original mutant from EEC, the testing of diverse value can't produce a bug in the model prediction. Hence, we conclude that adding more value isn't helpful in finding more fairness bug 

% \vspace{0.2cm}\noindent\textbf{RQ3. } {\em How good is Gender\toolname{} in generating bias-uncovering test cases?}

% From 25,000 texts in IMDB test set, Gender\toolname{} generated 3,730 templates and 986,752 mutants in total. Table~\ref{tab:stat-gender-mutant} details the mutants by the set of placeholders involved in their generation. From these mutants, Gender\toolname{} can generate 229,096 BTCs.

% \begin{table}[H]
%     \centering
%     \caption{Number of Gender Mutant Text}\ft{I am not sure if this is interesting. How many BTCs are there for each Placeholder Type? }
%     \begin{tabular}{ lcc }
%     \hline
%     \textbf{Placeholder Type} & \textbf{\# Templates} & \textbf{\# Mutants} \\
%     \hline
%     $\langle name \rangle$ & 3,047 & 944,570  \\
%     $\langle sltn-identifier\rangle$ $\langle name\rangle$ & 62 & 19,220 \\
%     $\langle gaw\rangle$ & 583 & 15,158 \\
%     $\langle pro\rangle$, $\langle name\rangle$ & 23 & 7,130  \\
%     $\langle pro\rangle$, $\langle sltn-identifier\rangle$ $\langle name\rangle$ & 1 & 310 \\
%     $\langle pro\rangle$, $\langle gaw\rangle$ & 14 & 364 \\
%     \hline
%     \textbf{Total} & \textbf{3,730}  & \textbf{986,752} \\
%     \hline
%     \end{tabular}
%     \label{tab:stat-gender-mutant}
% \end{table}
% \mh{The last 3 are Case 4}

% %The mutant then is inputted to fine-tuned BERT. The Table~\ref{tab:performance} shows the number of discordant pairs, FPED, and FNED.

% \dl{We need to show the intermediary statistics, e.g., how many males, how many females, etc.}

\begin{table}[H]
    \centering
    \caption{\toolname{}'s Performance in Finding Fairness Bugs}
    \begin{tabular}{ lc }
    \hline
    \textbf{Target Bias} & \textbf{\# BTC} \\
    \hline
    Gender & 71,027  \\
    Occupation & 109,386 \\
    Country-of-Origin & 18,182 \\
    Age & 107 \\
    \hline
    % \multicolumn{4}{l}{BTC: Bias-uncovering Test Cases}\\
    \end{tabular}
    \label{tab:performance}
\end{table}

% \begin{table}[H]
%     \centering
%     \caption{\toolname{}'s Performance in Finding Fairness Bugs}
%     \begin{tabular}{ lccc }
%     \hline
%     \textbf{Target Bias} & \textbf{FPED} & \textbf{FNED} & \textbf{\# BTC} \\
%     \hline
%     Gender & 0.00277 & 0.00343 & 229,096  \\
%     Occupation & 0.02635 & 0.04305 & 37,946 \\
%     Country-of-Origin & 0.01193 & 0.01861 & 240,192 \\
%     Age & 0.00034 & 0.00115 & 31 \\
%     \hline
%     % \multicolumn{4}{l}{BTC: Bias-uncovering Test Cases}\\
%     \end{tabular}
%     \label{tab:performance}
% \end{table}


%\section{Experiments on Other GenderBias Instances}



